Governmental incentives for green bonds investment

Motivated by the recent studies on the green bond market, we build a model in which an investor trades on a portfolio of green and conventional bonds, both issued by the same governmental entity. The government provides incentives to the bondholder in order to increase the amount invested in green bonds. These incentives are, optimally, indexed on the prices of the bonds, their quadratic variation and covariation. We show numerically on a set of French governmental bonds that our methodology outperforms the current tax-incentives systems in terms of green investments. Moreover, it is robust to model specification for bond prices and can be applied to a large portfolio of bonds using classical optimisation methods.

==> poubelle.tex <==



\section{Solving the investor's problem}

We take the special case of the absence of an exchange ($\xi=0$) and assume a CRRA utility function, that is $U(x)=x^{\gamma}$. For sake of rea, we omit the dependencies of the short rate coefficients with respect to time. The HJB equation associated to this stochastic control problem is given by
\begin{align*}
    & 0 = \partial_t v + \sup_\pi\bigg\{ \big(\pi (r^{i,g} + \xi^{i,g} \sigma^{i,g}) + (1 - \pi)(r^{j,c} + \xi^{j,c} \sigma^{j,c})\big) x v_x + \frac{1}{2}\big((\pi \sigma^{i,g})^2 + \big((1-\pi)\sigma^{j,c}\big)^2 + 2\rho \pi (1-\pi)\sigma^{i,g} \sigma^{j,c} \big)x^2 \partial_{xx}v \\
    & + a^{i,g} \partial_{r^{i,g}}v + a^{j,c} \partial_{r^{j,c}}v + \frac{1}{2}(b^{i,g})^2 \partial_{r^{i,g} r^{i,g}}v + \frac{1}{2}(b^{j,c})^2 \partial_{r^{j,c} r^{j,c}}v +  \rho b^{i,g} b^{j,c} \partial_{r^{j,c} r^{i,g}}v + b^{i,g} (\pi \sigma^{i,g} + \rho (1-\pi)\sigma^{j,c}) x \partial_{x r^{i,g}} v  \\
    & + b^{j,c} \big( (1-\pi)\sigma^{j,c}  + \rho \pi \sigma^{i,g}  \big) x \partial_{x r^{j,c}} v\bigg\}
\end{align*}
with terminal condition $v(T,x,r^{i,g},r^{j,c})=x^{\gamma}$. 


First order condition leads to
\begin{align*}
    & \pi^\star = -\frac{1}{x\partial_{xx}v \beta}\big(\beta^x \partial_x v + \beta^{r^{j,c} x} \partial_{r^{j,c} x} v + \beta^{r^{i,g} x}\partial_{r^{i,g} x} v\big) - \alpha^{cg}.
\end{align*}
where
\begin{align*}
    & \beta^x = r^{i,g} + \xi^{i,g} \sigma^{i,g} - r^{j,c} - \xi^{j,c} \sigma^{j,c}, \quad \beta^{r^{j,c} x} = b^{j,c} (\rho \sigma^{i,g} -\sigma^{j,c}),  \beta^{r^{i,g} x} = b^{i,g} (\sigma^{i,g} - \rho \sigma^{j,c}), \quad \beta = (\sigma^{j,c})^2 - 2\rho\sigma^{j,c} \sigma^{i,g} +(\sigma^{i,g})^2
\end{align*}
and 
$$
 \alpha^{cg}= \frac{\rho\sigma^{j,c}\sigma^{i,g} - (\sigma^{j,c})^2}{\beta}.
$$
By using the ansatz $v(t,x,r^{i,g},r^{j,c})=x^\gamma f(t,r^{i,g},r^{j,c})$, we get the PDE
\begin{align*}
     0 = & f \mu^t \partial_t f + f^2 \tilde{\mu}^{f^2} + f \tilde{\mu}^{r^{j,c} f} \partial_{r^{j,c}}f + f \tilde{\mu}^{r^{i,g} f} \partial_{r^{i,g}}f + f \mu^{r^{j,c} r^{j,c}} \partial_{r^{j,c} r^{i,g}}f + \tilde{\mu}^{r^{j,c}, r^{i,g}} \partial_{r^{j,c}}f  \partial_{r^{i,g}}f \\
    & + (\partial_{r^{j,c}}f)^2 \tilde{\mu}^{(r^{j,c})^2} + (\partial_{r^{i,g}}f)^2 \tilde{\mu}^{(r^{i,g})^2} + f \mu^{r^{j,c} r^{j,c}} \partial_{r^{j,c} r^{j,c}}f + f \mu^{r^{i,g} r^{i,g}} \partial_{r^{i,g} r^{i,g}}f
\end{align*}
with terminal condition $f(T,r^{j,c},r^{i,g})=1$, where
\begin{align*}
    & \tilde{\mu}^{f^2} = -\frac{(\beta^x)^2 \gamma^2}{2\beta} + \gamma^2(\gamma-1)(r^{j,c} + \xi^{j,c} \sigma^{j,c}) + \frac{1}{2}\gamma^2 (\gamma-1)^2 (\sigma^{j,c})^2  + \gamma^2(\gamma-1) \big(\rho\sigma^{j,c}\sigma^{i,g} -(\sigma^{j,c})^2\big)\beta^x \frac{\beta - 1}{\beta} \\
    & - \gamma^2(\gamma-1)^2 (\rho\sigma^{j,c}\sigma^{i,g} - (\sigma^{j,c})^2) -\gamma^2(\gamma-1)\beta^x + \frac{1}{2}\gamma^2(\gamma-1)^2 (\alpha^{cg})^2 \beta , \\
    & \tilde{\mu}^{r^{j,c} f} =   \gamma(\gamma-1)a^{j,c} + b^{j,c} \sigma^{j,c} \gamma^2 (\gamma-1) + \beta^{r^{j,c} x}\beta^x\gamma^2   + \gamma^2(\gamma-1)\beta^{r^{j,c} x} \big( \alpha^{cg} - 1 + \rho\sigma^{j,c}\sigma^{i,g} -(\sigma^{j,c})^2 \big)\\
    & \tilde{\mu}^{r^{i,g} f} =  \gamma(\gamma-1)a^{i,g} + b^{i,g} \rho \sigma^{j,c} \gamma^2 (\gamma-1)  + \beta^{r^{i,g} x}\beta^x\gamma^2  + \gamma^2(\gamma-1)\beta^{r^{i,g} x}\big( \alpha^{cg} -1 + \rho\sigma^{j,c} \sigma^{i,g} -(\sigma^{j,c})^2 \big)\\
    & \tilde{\mu}^{r^{i,g},r^{j,c}} = - \frac{\gamma^2\beta^{r^{j,c} x}\beta^{r^{i,g} x}}{\beta} \\
    & \tilde{\mu}^{(r^{j,c})^2}= (\beta^{r^{j,c} x})^2\gamma^2 + \frac{(\beta^{r^{j,c} x})^2\gamma^2}{2\beta} \\
    & \tilde{\mu}^{(r^{i,g})^2}= (\beta^{r^{i,g} x})^2\gamma^2 + \frac{(\beta^{r^{i,g} x})^2\gamma^2}{2\beta} \\
    & \mu^{r^{j,c} r^{j,c}}= \frac{1}{2}\gamma(\gamma-1)(b^{j,c})^2 \\
    & \mu^{r^{i,g} r^{i,g}}= \frac{1}{2}\gamma(\gamma-1)(b^{i,g})^2 \\
    & \mu^{r^{i,g} r^{j,c}}=\rho\sigma^{i,g}\sigma^{j,c} \gamma(\gamma-1). 
\end{align*}
We now make another ansatz: $$f(t,r^{i,g},r^{j,c})=g(t)\exp\big(\kappa^{i,g}_t r^{i,g} + \kappa^{j,c}_t r^{j,c} + \kappa^{gg}_t (r^{i,g})^2 + \kappa^{cc}_t (r^{j,c})^2 + \kappa^{gc}_t r^{i,g} r^{j,c}\big).$$
with terminal conditions $g(T)=1, \kappa^{i,g}_T = \kappa^{j,c}_T = \kappa^{gg}_T = \kappa^{cc}_T = \kappa^{gc}_T =0$. 
This leads to the following PDE:
\begin{align*}
    & 0 = g\Big[ (r^{j,c})^2 C^{cc}_t + (r^{i,g})^2 C^{gg}_t + (r^{i,g} r^{j,c}) C^{cg}_t + r^{j,c} C^{c}_t + r^{i,g} C^{g}_t  \Big] \\
    & + g \Big[ \kappa_t^{j,c} \tilde{C}^{r^{j,c} f} + \kappa_t^{i,g} \tilde{C}^{r^{i,g} f} + (\kappa_t^{gc} + \kappa_t^{i,g} \kappa_t^{j,c})\mu^{r^{i,g} r^{j,c}} + (\kappa_t^{i,g} \kappa_t^{j,c})\tilde{\mu}^{r^{i,g},r^{j,c}} + (\kappa_t^{j,c})^2 \tilde{\mu}^{(r^{j,c})^2} + (\kappa_t^{i,g})^2 \tilde{\mu}^{(r^{i,g})^2} \\
    & + (2\kappa_t^{cc} + (\kappa_t^{j,c})^2)\mu^{r^{j,c} r^{j,c}} + (2\kappa_t^{gg} + (\kappa_t^{i,g})^2)\mu^{r^{i,g} r^{i,g}} + \tilde{C}^{f^2}  \Big] + \partial_t g
\end{align*}
\begin{color}{red}
 Les calculs pour la solution explicites étaient vraiment très longs (je peux t'envoyer les résultats que j'ai sur mes feuilles de brouillon si tu veux?). Les $C_t$ dépendent des fonctions $\kappa$ et pour supprimer le terme de la première ligne j'ai un système de 5 ODE (couplées). \\
 
Ensuite je réinjecte la forme des $\kappa$ dans ce qu'il reste de l'équation et j'ai une ODE en $g$ où je n'ai plus que le temps comme dimension. Je voulais juste avoir ton avis sur le fait que j'ai été obligé d'utiliser un ansatz comme celui la car je me retrouve avec des termes en $r^{i,g},r^{j,c}$ d'ordre 2 (peut être car les taux sont corrélés?). Est ce que cela te parait cohérent? \\
 
Si ce que j'ai fais est juste, on a une solution explicite dans ce cas. 
\end{color}











\section{Solving the Agent's problem}

We define the set of contractible variable as $B^\pi = (X^\pi,r^{i,g},r^{j,c})$, and for notational simplicity we set
\begin{align*}
   & dX_t = K^{x,t}(t,B_t^\pi) dt + K^{x,g}(t,B_t^\pi)dW_t^{i,g} + K^{x,c}(t,B_t^\pi)dW_t^{j,c},  \\
   & dr_t^{i,g} = K^{g,t}(t,B_t^\pi) dt + b^{i,g} dW_t^{i,g}, \\
   & dr_t^{j,c} = K^{c,t}(t,B_t^\pi) dt + b^{j,c} dW_t^{j,c}. 
\end{align*}
For sake of readability, we will omit the dependence with respect to the set of contractible variables $B^\pi$. We define the covariation matrix of the contractible variables as
\begin{align*}
\langle B^\pi \rangle_t = 
    \begin{pmatrix}
    (K_t^{x,g})^2 + (K_t^{x,c})^2 + 2\rho K_t^{x,g} K_t^{x,c} & b^{i,g} (K_t^{x,g}+\rho K_t^{x,c}) & b^{j,c} (K_t^{x,c} + \rho K_t^{x,g}) \\
    b^{i,g} (K_t^{x,g}+\rho K_t^{x,c}) & (b^{i,g})^2 & \rho b^{i,g} b^{j,c} \\
    b^{j,c} (K_t^{x,c} + \rho K_t^{x,g}) & \rho b^{i,g} b^{j,c} & (b^{j,c})^2
    \end{pmatrix}.
\end{align*}

We define,
\begin{align*}
    J(\tau,\pi) = \mathbb{E}_\tau\big[ -\exp\big(-\gamma(X_T^\pi - X_\tau^\pi +\xi)\big)\big], \quad V_\tau = \sup_\pi J(\tau,\pi),
\end{align*}
and introduce the following dynamic programming principle:
\begin{align*}
    V^A (t,B_t) = \sup_\pi \mathbb{E}_t\Big[ -\exp\big(-\gamma(X_\tau^\pi - X_t^\pi)\big)V_\tau\Big].
\end{align*}
Assume the function $V^A$ is smooth enough, then there exist predictable processes 
\begin{align*}
    \tilde{Z} = \big(\tilde{Z}^x, \tilde{Z}^{i,g}, \tilde{Z}^{j,c} \big), \quad \tilde{\Gamma} = 
    \begin{pmatrix}
     \tilde \Gamma^x & \tilde \Gamma^{x,g} & \tilde \Gamma^{x,c} \\
     \tilde \Gamma^{x,g} & \tilde \Gamma^{i,g} & \tilde \Gamma^{g,c} \\
     \tilde \Gamma^{x,c} & \tilde \Gamma^{g,c} & \tilde \Gamma^ c
    \end{pmatrix},
\end{align*}
such that
\begin{align*}
    dV^A(t,B_t^\pi) &=  \partial_t V^A (t,B_t^\pi) dt + \frac{1}{2}\text{Tr}\big(\tilde{\Gamma}_t d\langle B^\pi \rangle_t\big) + \tilde Z_t \cdot dB_t^\pi \\ 
     & =\Big(\partial_t V^A (t,B_t^\pi) + \tilde{Z}_t^x K_t^{x,t} + \tilde{Z}_t^{i,g} K^{g,t}(t) + \tilde{Z}_t^{j,c} K^{c,t}(t) + \frac{1}{2}\tilde{\Gamma}_t^x \big((K_t^{x,g})^2 + (K_t^{x,c})^2 + 2\rho K_t^{x,g}K_t^{x,c}\big) \\
   & + \frac{1}{2}\tilde{\Gamma}_t^{i,g} (b^{i,g})^2 + \frac{1}{2}\tilde{\Gamma}_t^{j,c} (b^{j,c})^2 + \tilde{\Gamma}_t^{x,g} b^{i,g} (K_t^{x,g}+\rho K_t^{x,c}) + \tilde{\Gamma}_t^{x,c} b^{j,c} (K_t^{x,c}+\rho K_t^{x,g}) + \tilde{\Gamma}_t^{g,c} \rho b^{i,g} b^{j,c} \Big) dt \\
   & + \big( \tilde{Z}_t^x K_t^{x,g} + \tilde{Z}_t^{i,g} b^{i,g}\big) dW_t^{i,g} +  \big( \tilde{Z}_t^x K_t^{x,c} + \tilde{Z}_t^{j,c} b^{j,c}\big) dW_t^{j,c}.
\end{align*}
By Ito's formula we have
\begin{align*}
    \frac{d \exp(-\gamma X_t^\pi)}{\exp(-\gamma X_t^\pi)} = & \Big( -\gamma K_t^{x,t} + \frac{\gamma^2}{2} \big( (K_t^{x,g})^2 + (K_t^{x,c})^2 + 2\rho K_t^{x,g} K_t^{x,c} \big)\Big) dt \\
    & - \gamma K_t^{x,g}dW_t^{i,g} - \gamma K_t^{x,c} dW_t^{j,c} \\
    & := K_t^{e,t} dt + K_t^{e,g} dW_t^{i,g} + K_t^{e,c}dW_t^{j,c}.
\end{align*}
From the martingale representation theorem and the dynamic programming principle, the process $V^A(t,B_t^\pi)\exp(-\gamma X_t^\pi)$ should be a supermartingale for all $\pi\in \mathcal{A}$, and a martingale for the optimal control $\pi^\star$. By Ito's formula, equalling the drift of $V^A(t,B_t^\pi)\exp(-\gamma X_t^\pi)$ to zero we have
\begin{align*}
    0 = -\partial_t V^A (t,B_t^\pi) + \gamma V(t,B^\pi_t) G(t,Z_t,\Gamma_t,B_t^\pi)
\end{align*}
where $(Z_t,\Gamma_t) = -\frac{1}{\gamma V^A(t,B_t^\pi)}(\tilde{Z}_t, \tilde{\Gamma}_t)$ and
\begin{align*}
    G(t,Z_t,\Gamma_t,B_t^\pi)= & \sup_\pi \bigg\{ -\frac{K_t^{e,t}}{\gamma} + Z_t^x K_t^{x,t} + Z_t^{j,c} K^{c,t}(t) + Z_t^{i,g} K^{g,t}(t) + \frac{1}{2}\Gamma_t^x \big( (K_t^{x,g})^2 + (K_t^{x,c})^2 + 2\rho K_t^{x,g} K_t^{x,c}\big) \\
    & + \frac{1}{2}\Gamma_t^{i,g} (b^{i,g})^2 + \frac{1}{2}\Gamma_t^{j,c} (b^{j,c})^2 + \Gamma_t^{x,g}b^{i,g} (K_t^{x,g}+\rho K_t^{x,c}) + \Gamma_t^{x,c}b^{j,c} (K_t^{x,c}+\rho K_t^{x,g}) + \Gamma_t^{g,c}\rho b^{i,g} b^{j,c} \\
    & + K_t^{e,g}\big( Z_t^x K_t^{x,g} + Z_t^{i,g} b^{i,g} + \rho (Z_t^x K_t^{x,c}+Z_t^{j,c} b^{j,c})\big) + K_t^{e,c}\big( Z_t^x K_t^{x,c} + Z_t^{j,c} b^{j,c} + \rho (Z_t^x K_t^{x,g}+Z_t^{i,g} b^{i,g})\big)   \bigg\}.
\end{align*}
We define the following form of contract:
\begin{align*}
    \xi = Y_T^{Y_0,Z,\Gamma} =&  Y_0 + \int_0^T Z_t^x dX_t + Z_t^{j,c} dr_t^{j,c} + Z_t^{i,g} dr_t^{i,g} + \frac{1}{2} \Gamma_t^x d\langle X \rangle_t + \frac{1}{2} \Gamma_t^{i,g} d\langle r^{i,g} \rangle_t + \frac{1}{2} \Gamma_t^{j,c} d\langle r^{j,c} \rangle_t + \Gamma_t^{x,c} d\langle X, r^{j,c} \rangle_t \\
    & \Gamma_t^{x,g} d\langle X, r^r \rangle_t + \Gamma_t^{g,c} d\langle r^{i,g}, r^{j,c} \rangle_t +\bigg( \frac{\gamma}{2}\Big( (K_t^{x,g}Z_t^x +Z_t^{i,g} b^{i,g})^2 + (K_t^{x,c}Z_t^x + Z_t^{j,c} b^{j,c})^2 \\
    & + 2\rho (K_t^{x,g}Z_t^x +Z_t^{i,g} b^{i,g})(K_t^{x,c}Z_t^x + Z_t^{j,c} b^{j,c})\Big) - G(t,Z_t,\Gamma_t,B_t^\pi)\bigg) dt. 
\end{align*}
In matrix form, it rewrites as
\begin{align*}
    \xi = Y_T^{Y_0,Z,\Gamma} =& Y_0 + \int_0^T Z_t \cdot dB_t^\pi + \frac{1}{2}\text{Tr}\Big(\big(\Gamma_t + \gamma Z_t Z_t^\top\big)d\langle B^\pi \rangle_t \Big) - G(t,Z_t,\Gamma_t,B_t^\pi) dt. 
\end{align*}
We can directly check that the process $\exp\big(-\gamma (X_t + Y_t)\big)$ is a martingale when $\pi=\pi^\star$. Finally, the optimal control of the asset manager is given by
\begin{align*}
    \pi^\star_t = -\frac{Z_t^{i,g} \alpha_t^{i,g} + Z_t^{j,c} \alpha_t^{j,c} + \Gamma_t^{x,g}\alpha_t^{x,g} + \Gamma_t^{x,c}\alpha_t^{x,c} + Z_t^x \alpha_t^x + \Gamma_t^x \alpha_t^{xx} + \big(\beta_t + \gamma X_t \big( (\sigma_t^{j,c})^2 -\rho\sigma^{j,c}\sigma^{i,g}\big) \big) }{\big((\sigma_t^{i,g})^2 + (\sigma_t^{j,c})^2 -2\rho\sigma^{j,c}_t \sigma^{i,g}_t \big) X_t (\Gamma_t^x -\gamma -2\gamma Z_t^x)},
\end{align*}
where
\begin{align*}
    & \alpha^{i,g} = \gamma b^{i,g} (\rho\sigma^{j,c} -\sigma^{i,g}), \quad \alpha^{j,c} = \gamma b^{j,c} (\sigma^{j,c} - \rho\sigma^{i,g}) , \quad \alpha^{x,g}= b^{i,g} (\sigma^{i,g} - \rho\sigma^{j,c}), \quad  \alpha^{x,c}= b^{j,c} (\rho\sigma^{i,g} - \sigma^{j,c}), \\
    & \alpha^x = \beta + 2\gamma x \big( (\sigma^{j,c})^2 -\rho\sigma^{j,c}\sigma^{i,g}\big), \quad \alpha^{xx} =  x \big(\rho\sigma^{j,c}\sigma^{i,g} -(\sigma^{j,c})^2 \big), \quad \beta = r^{i,g} + \xi^{i,g}\sigma^{i,g} -r^{j,c}-\xi^{j,c}\sigma^{j,c}. 
\end{align*}


\section{Solving the Principal's problem}

We define the following state process:
\begin{align*}
    \tilde{Y}_T^{Y_0,Z,\Gamma} =& Y_0 + \int_0^T Z_t \cdot dB_t^\pi + \frac{1}{2}\text{Tr}\Big(\big(\Gamma_t + \gamma Z_t Z_t^\top\big)d\langle B^\pi \rangle_t \Big) - \big( G(t,Z_t,\Gamma_t,B_t^\pi) + (G-\pi_t^\star)^2 \big)  dt. \\
    & := Y_0 + \int_0^T K_t^{y,t}dt + K_t^{y,g}dW_t^{i,g} + K_t^{y,c}dW_t^{j,c}.
\end{align*}
The Hamilton-Jacobi-Bellman equation associated to the Principal's problem can be written as:
\begin{align*}
    0 = & \partial_t v +\sup_{z,\Gamma}\bigg\{ K_t^{x,t} \partial_x v + \frac{1}{2}\partial_{xx}v \big((K^{x,g}_t)^2 + (K^{x,c}_t)^2  + 2\rho K^{x,g}_t K^{x,c}_t\big) + \partial_{r^{i,g}}v K^{g,t}(t) + \frac{1}{2}\partial_{r^{i,g} r^{i,g}}v (b^{i,g})^2 \\
    & \partial_{r^{j,c}}v K^{c,t}(t) + \frac{1}{2}\partial_{r^{j,c} r^{j,c}}v (b^{j,c})^2 + \partial_{\tilde y}v K_t^{y,t} + \frac{1}{2}\partial_{\tilde y \tilde y}v \big((K^{y,g}_t)^2 + (K^{y,c}_t)^2  + 2\rho K^{y,g}_t K^{y,c}_t\big) \\
    & \partial_{r^{i,g} x}v b^{i,g} (K_t^{x,g}+\rho K_t^{x,c}) + \partial_{r^{j,c} x}v b^{j,c} (K_t^{x,c}+\rho K_t^{x,g}) + \partial_{r^{i,g} r^{j,c}}v \rho b^{j,c} b^{i,g} \\ 
    & + \partial_{xy}v \big( K_t^{x,g}(K_t^{y,g}+\rho K_t^{y,c}) + K_t^{x,c}(K_t^{y,c}+\rho K_t^{y,g})\big) \\
    & \partial_{r^{i,g} \tilde{y}}v b^{i,g} (K_t^{y,g}+\rho K_t^{y,c}) + \partial_{r^{j,c} y}v b^{j,c} (K_t^{y,c}+ \rho K_t^{y,g})\bigg\},
\end{align*}
with terminal condition $v(T,x,r^{i,g},r^{j,c},\tilde{y})=-\exp(\eta \tilde{y})$. We use the ansatz 
\begin{align*}
    v(T,x,r^{i,g},r^{j,c},\tilde{y})=u(t,x,r^{i,g},r^{j,c})\exp(\eta \tilde{y}), \quad u(T,x,r^{i,g},r^{j,c})=-1,
\end{align*}
which leads to
\begin{align*}
   0 = & \partial_t u +\sup_{z,\Gamma}\bigg\{ \partial_t u + K_t^{x,t} \partial_x v + \frac{1}{2}\partial_{xx}v \big((K^{x,g}_t)^2 + (K^{x,c}_t)^2  + 2\rho K^{x,g}_t K^{x,c}_t\big) + \partial_{r^{i,g}}v K^{g,t}(t) + \frac{1}{2}\partial_{r^{i,g} r^{i,g}}v (b^{i,g})^2 \\
    & \partial_{r^{j,c}}v K^{c,t}(t) + \frac{1}{2}\partial_{r^{j,c} r^{j,c}}v (b^{j,c})^2 + \eta v K_t^{y,t} + \frac{1}{2}\eta^2 v \big((K^{y,g}_t)^2 + (K^{y,c}_t)^2  + 2\rho K^{y,g}_t K^{y,c}_t\big) \\
    & \partial_{r^{i,g} x}v b^{i,g} (K_t^{x,g}+\rho K_t^{x,c}) + \partial_{r^{j,c} x}v b^{j,c} (K_t^{x,c}+\rho K_t^{x,g}) + \partial_{r^{i,g} r^{j,c}}v \rho b^{j,c} b^{i,g} \\ 
    & + \eta \partial_{x}v \big( K_t^{x,g}(K_t^{y,g}+\rho K_t^{y,c}) + K_t^{x,c}(K_t^{y,c}+\rho K_t^{y,g})\big) \\
    & \eta \partial_{r^{i,g} }v b^{i,g} (K_t^{y,g}+\rho K_t^{y,c}) + \eta \partial_{r^{j,c} }v b^{j,c} (K_t^{y,c}+ \rho K_t^{y,g})\bigg\}.
\end{align*}
This $3$-dimensional HJB equation can easily be solved numerically to derive the incentives of the Principal. 








We work on the canonical space $\Omega$ of continuous functions on $[0,T]$, with its Borel sigma algebra $\mathcal{F}$. We define the canonical process 
\begin{align*}
    \mathcal{X}_t = \big(X_t,W_t^c,W_t^g,W_t^I\big)\in \mathbb{R}\times \mathbb{R}^{d^c}\times \mathbb{R}^{d^g}\times\mathbb{R}= \mathbb{R}^{\mathcal{D}},
\end{align*}
and its natural filtration $\mathbb{F}=(\mathcal{F}_t)_{t\geq 0}$. We set $\mathcal{F}=\mathcal{F}_T$ and $\mathbb{P}_0$ the $\mathcal{D}$-dimensional Wiener measure on $\Omega$. 







We define the value function of the investor at time $t$ as
\begin{align*}
    V^A(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi}) = \sup_\pi \mathbb{E}_t\Big[-\exp\big(-\gamma(\xi - K_T^\pi)\big)\Big]. 
\end{align*}
If this function is smooth enough, there exists predictable processes 

such that
\begin{align*}
    dV^A(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi}) & = \partial_t V^A(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi}) dt + \tilde{Z}_t^{\text{obs},\pi} dB_t^{\text{obs},\pi} + \tilde{Z}_t^{\cancel{\text{obs}},\pi} dB_t^{\cancel{\text{obs}},\pi} \\
    & + \frac{1}{2}\text{Tr}\big( \tilde{\Gamma}_t^{\text{obs},\pi} d\langle B^{\text{obs},\pi}\rangle_t \big)  + \frac{1}{2}\text{Tr}\big( \tilde{\Gamma}_t^{\cancel{\text{obs}},\pi} d\langle B^{\cancel{\text{obs}},\pi}\rangle_t \big) \\
    & + \text{Tr}\big( \tilde{\Gamma}_t^{\text{obs},\cancel{\text{obs}},\pi} d\langle B^{\text{obs},\pi}, B^{\cancel{\text{obs}},\pi}\rangle_t \big) \\
    & = \Big( \partial_t V^A(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi})+ \tilde{Z}_t^{\text{obs},\pi} \cdot \mu_t^{\text{obs},\pi} + \tilde{Z}_t^{\cancel{\text{obs}},\pi} \cdot \mu_t^{\cancel{\text{obs}},\pi} \\
    & +  \frac{1}{2}\text{Tr}\big( \tilde{\Gamma}_t^{\text{obs},\pi}\Sigma_t^{\text{obs},\pi}\Omega (\Sigma_t^{\text{obs},\pi})^{\top}  \big)  
    + \frac{1}{2}\text{Tr}\big( \tilde{\Gamma}_t^{\cancel{\text{obs}},\pi}\Sigma_t^{\cancel{\text{obs}},\pi}\Omega (\Sigma_t^{\cancel{\text{obs}},\pi})^{\top}   \big) \Big)dt \\
    & + \text{Tr}\big( \tilde{\Gamma}_t^{\text{obs},\cancel{\text{obs}},\pi}\Sigma_t^{\cancel{\text{obs}},\pi}\Omega (\Sigma_t^{\text{obs},\pi})^{\top} \big) \\
    & + \Big( (\Sigma_t^{\text{obs},\pi})^{\top} \tilde{Z}_t^{\text{obs},\pi} + (\Sigma_t^{\cancel{\text{obs}},\pi})^{\top} \tilde{Z}_t^{\cancel{\text{obs}},\pi}\Big) dW_t .
\end{align*}
Moreover,
\begin{align*}
    \frac{d \exp(\gamma K_T^\pi)}{\exp(\gamma K_T^\pi)} = \gamma k(\pi_t) dt.
\end{align*}
From the martingale representation theorem and the dynamic programming principle, the process
\begin{align*}
    V^A(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi})\exp(\gamma K_T^\pi)
\end{align*}
should be a supermartingale for all $\pi\in \mathcal{A}$, and a martingale for the optimal control $\pi^\star$. By Ito's formula, equalling the drift of $V^A(t,B_t^\pi)\exp(\gamma K_T^\pi)$ to zero we have
\begin{align*}
    0 = -\partial_t V^A (t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi}) + \gamma V(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi}) G(t,Z_t,\Gamma_t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}}}),
\end{align*}
where $(Z_t,\Gamma_t) = -\frac{1}{\gamma V^A(t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}},\pi})}(\tilde{Z}_t, \tilde{\Gamma}_t)$ and
\begin{align*}
    G(t,Z_t,\Gamma_t,B_t^{\text{obs},\pi},B_t^{\cancel{\text{obs}}})= & \sup_\pi \bigg\{ -k(\pi_t) + Z_t^{\text{obs},\pi} \cdot \mu_t^{\text{obs},\pi} + Z_t^{\cancel{\text{obs}},\pi} \cdot \mu_t^{\cancel{\text{obs}},\pi} \\
    & + \frac{1}{2}\text{Tr}\big( \Gamma^{\text{obs},\pi}\Sigma_t^{\text{obs},\pi}\Omega (\Sigma_t^{\text{obs},\pi})^{\top}  \big) + \frac{1}{2}\text{Tr}\big( \Gamma^{\cancel{\text{obs}},\pi}\Sigma_t^{\cancel{\text{obs}},\pi}\Omega (\Sigma_t^{\cancel{\text{obs}},\pi})^{\top}  \big) \\
    & + \text{Tr}\big( \Gamma^{\text{obs},\cancel{\text{obs}},\pi}\Sigma_t^{\cancel{\text{obs}},\pi}\Omega(\Sigma_t^{\text{obs},\pi})^{\top}  \big)
   \bigg\}.
\end{align*}

From the definition of $G$, we see that the expression of the contract does not depend on $\tilde \Gamma^{\cancel{\text{obs}},\pi}$ and $\Gamma^{\text{obs},\cancel{\text{obs}},\pi}$. We also expect that the contract does not depend on $Z_t^{\cancel{\text{obs}}}$, that is $Z_t^{\cancel{\text{obs}}}=0$. Therefore, we can state the definition of an admissible contract.













We define the Hamiltonian $H:[0,T]\times P^S \times \mathbb{R}^{2d^g+2}\times \mathbb{R}\times\mathbb{R}\times P^S \times \mathbb{R}^{d^g+2} \to \mathbb{R}$ as
\begin{align*}
    & H(t,z,g,b,v_q,v_{qq},v_b,v_{bb},v_{qb}) := v_q\Big( z\cdot \mu^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g),r^g\big) + \sum_{i=1}^{d^g}\big(G_i -\hat\pi_i(t,z,g,r^g)\big)^2 \\
    & + \frac{1}{2}\text{Tr}\Big[(g+\gamma z z^{\top})\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\big(\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\big)^{\top}\Big] \\
    &  - h^{\text{\rm obs},S}\big(t,z,g,r^g,\hat\pi(t,z,g,r^g)\big) \Big) + \frac{1}{2}\text{Tr}\bigg[ z^{\top} \Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Sigma\Big(\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)^{\top}z v_{qq}\Big)\bigg] \\
    & + v_b \cdot \mu^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g),r^g\big) + \frac{1}{2}\text{Tr}\Big[ \Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)(\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big))^{\top} v_{bb} \Big]  \\
    & + \text{Tr}\bigg[\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big(z\cdot \Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big)^{\top} v_{qb} \bigg], 
\end{align*}







\begin{equation*}
\begin{split}
\begin{cases}
   &  \partial_t V(t,b,q) + \underset{(z,g,\hat\pi)\in P^S \times \mathcal{O}^{\text{obs},S}}{\sup } H\big(t,z,g,b,V_q,V_{qq},V_b,V_{bb},V_{qb}\big) =0,\\
    & V(T,b,q)= -\exp(-\nu q),
\end{cases}
\end{split}
\end{equation*}
where $(t,b,q)\in [0,T)\times \mathbb{R}^{2d^g+2} \times \mathbb{R}$ and for all $(i,j)\in \{1,\dots,2d^g+2\}$, $(V_b)_i = \partial_{b_i} V, (V_{bb})_{i,j}=\partial_{b_i b_j}V$. We use the change of variable
\begin{align*}
    V(t,b,q)= U(t,b)\exp(-\nu q),
\end{align*}
such that the HJB equation becomes
\begin{align}\label{hjb_stoc_rates}
\begin{split}
\begin{cases}
   &  \partial_t U(t,b) + \underset{(z,g,\hat\pi)\in P^S \times \mathcal{O}^{\text{obs},S}}{\sup } \tilde{H}\big(t,z,g,b,U,U_b,U_{bb}\big) =0,\\
    & U(T,b)= -1,
\end{cases}
\end{split}
\end{align}
where $\tilde{H}:[0,T]\times P^S \times  \mathbb{R}\times P^S \to \mathbb{R}$ is defined by
\begin{align*}
    & \tilde{H}(t,z,g,u,u_b,u_{bb}) := \nu u  \bigg( z \cdot \mu^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g),r^g\big) +  \sum_{i=1}^{d^g}\big(G_i -\hat\pi_i^{g}(t,z,g,r^g)\big)^2 \\
    & + \frac{1}{2}\text{Tr}\bigg[(g+\gamma z z^{\top})\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big(\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big)^{\top}\bigg] - h^{\text{\rm obs},S}\big(t,z,g,r^g,\hat\pi(t,z,g,r^g)\big)  \bigg) \\
    & + \frac{1}{2} \nu^2 u \text{Tr}\bigg[z z^{\top} \Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big(\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big)^{\top}\bigg] + u_b \cdot \mu^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g),r^g\big) \\
    & + \frac{1}{2}\text{Tr}\bigg[ \Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big(\Sigma^{\text{\rm obs},S}\big(t,\hat\pi(t,z,g,r^g)\big)\Big)^{\top} u_{bb} \bigg].
\end{align*}
